Can We Make Code Green? Understanding Trade-Offs in LLMs vs. Human Code Optimizations

The rapid technological evolution has accelerated software development for various domains and use cases, contributing to a growing share of global carbon emissions. While recent large language models (LLMs) claim to assist developers in optimizing code for performance and energy efficiency, their efficacy in real-world scenarios remains under exploration. In this work, we explore the effectiveness of LLMs in reducing the environmental footprint of real-world projects, focusing on software written in Matlab-widely used in both academia and industry for scientific and engineering applications. We analyze energy-focused optimization on 400 scripts across 100 top GitHub repositories. We examine potential 2,176 optimizations recommended by leading LLMs, such as GPT-3, GPT-4, Llama, and Mixtral, and a senior Matlab developer, on energy consumption, memory usage, execution time consumption, and code correctness. The developer serves as a real-world baseline for comparing typical human and LLM-generated optimizations. Mapping these optimizations to 13 high-level themes, we found that LLMs propose a broad spectrum of improvements--beyond energy efficiency--including improving code readability and maintainability, memory management, error handling while the developer overlooked some parallel processing, error handling etc. However, our statistical tests reveal that the energy-focused optimizations unexpectedly negatively impacted memory usage, with no clear benefits regarding execution time or energy consumption. Our qualitative analysis of energy-time trade-offs revealed that some themes, such as vectorization preallocation, were among the common themes shaping these trade-offs. With LLMs becoming ubiquitous in modern software development, our study serves as a call to action: prioritizing the evaluation of common coding practices to identify the green ones.

==> Listings/Optimized-code-GPT-4o.tex <==
%\footnote{\url{}}
\begin{minipage}{0.90\linewidth}
    \begin{lstlisting}[caption={The optimization of PSO Function by \gpt-4},
     label={optiimized-PSO-function-gpt4}]
% Define common parameters

fitnessFunc = @fitness;
w = 0.5;  % inertia weight
maxIter = 100;  % maximum number of iterations
popSizeArray = [50, 100, 500];
c1 = 1.5;
c2 = 1.5;
dim = 30;  % dimension size


% Initializing results storage

xm = cell(1, numel(popSizeArray));
fv = cell(1, numel(popSizeArray));

% Loop through different population sizes

for idx = 1:numel(popSizeArray)
    popSize = popSizeArray(idx);
    [xm{idx}, fv{idx}] = PSO(fitnessFunc, popSize, c1, c2, w, maxIter, dim);
end

% Access results if needed
xm1 = xm{1};
fv1 = fv{1};
xm2 = xm{2};
fv2 = fv{2};
xm3 = xm{3};
fv3 = fv{3};

\end{lstlisting}
\end{minipage}

==> Listings/Reasoning-optimized-code-GPT-3.tex <==
\begin{minipage}{0.90\linewidth}
    \begin{lstlisting}[caption={The reasoning for the PSO Function by \gpt-3},
     label={reasoning-PSO-function-gpt3}]
Reasoning for the optimization:
1. **Parameterization**: By storing the varying parameters in arrays, we can reduce code duplication and make it easier to modify the parameters in the future.
2. **Loop Optimization**: Instead of repeating the same code with different parameters multiple times, we can use a loop to iterate over the parameters and optimize the code execution.
3. **Efficiency**: This refactored code reduces redundancy, making it more concise and easier to maintain. It also minimizes the number of function calls to `PSO`, potentially improving energy efficiency during execution.
\end{lstlisting}
\end{minipage}

==> Listings/Reasoning-optimized-code-GPT-4.tex <==
\begin{minipage}{0.90\linewidth}
    \begin{lstlisting}[caption={The reasoning for the PSO Function by \gpt-4},
     label={reasoning-PSO-function-gpt4}]
**Reasoning for the Optimization:**

1. **Parameter Consolidation:** The code contains several repeated parameters for the `PSO` function calls. Consolidating these parameters into variables reduces redundancy and makes the code easier to maintain and modify.

2. **Looping Structure:** Instead of calling the `PSO` function multiple times manually, a loop is used to iterate over an array of particle numbers. This reduces code repetition and enhances scalability.

3. **Cell Array Storage:** The results from each `PSO` call are stored in a cell array, which allows for easy access and assignment to the final variables.

These changes improve the code's readability, maintainability, and potentially reduce the energy consumption by minimizing repeated variable initialization and redundant function calls.
\end{lstlisting}
\end{minipage}

==> Listings/non-optimized-code.tex <==
%\footnote{\url{}}
% Listing from the project ./../resource/sampling/repos_projects_filtered_top100stars/Smart-Algorithm/Particle_Swarm_Optimization/PSO-basic/main.m
\begin{minipage}{0.90\linewidth}
    \begin{lstlisting}[caption={Examplary injected code in a prompt, e.g., \autoref{lst:Prompt-llm}},
     label={lst:non-optiimized-PSO-function}]
clear
clc
% [xm1, fv1] = PSO(@fitness, 50, 1.5, 2.5, 0.5, 100, 30);
% [xm2, fv2] = PSO(@fitness, 50, 1.5, 2.5, 0.5, 1000, 30);
% [xm3, fv3] = PSO(@fitness, 50, 1.5, 2.5, 0.5, 10000, 30);

% [xm1, fv1] = PSO(@fitness, 50, 1.5, 2.5, 0.5, 100, 30);
% [xm2, fv2] = PSO(@fitness, 100, 1.5, 2.5, 0.5, 100, 30);
% [xm3, fv3] = PSO(@fitness, 200, 1.5, 2.5, 0.5, 100, 30);

[xm1, fv1] = PSO(@fitness, 50, 1.5, 1.5, 0.5, 100, 30);
[xm2, fv2] = PSO(@fitness, 100, 1.5, 1.5, 0.5, 100, 30);
[xm3, fv3] = PSO(@fitness, 500, 1.5, 1.5, 0.5, 100, 30);
\end{lstlisting}
\end{minipage}

==> Tables/Comprision-optimization-themes.tex <==
\begin{table*}
\scriptsize
\centering
		\caption{Common optimization themes (by LLMs and the developer) based on positive and negative performance delta (PD=original-optimized)}
  \label{tab:performance-optimization-themes}
		\begin{tabular}{p{0.07\linewidth}p{0.1\linewidth}p{0.7\linewidth}}			\toprule
       \textbf{PD} & \textbf{Metric} & \textbf{Themes}  \\ 
     \midrule
Positive (top quartile) & Energy & Vectorization, Improved Memory Management, Logical Indexing, Removed Unnecessary Code \\
\midrule
 & Time & Loop Optimization, Efficient Indexing, Removed Redundant Code, Improved Parallelization \\
\midrule
 & Memory & Preallocation, Vectorization, Removal of Unnecessary Variables, Optimized Data Structures \\
\midrule

Negative (bottom quartile) & Energy & Inefficient Memory Use, Unoptimized Loops, Complex Logic or transformation\\
\midrule
 & Time & Nested Loops, Unoptimized Logic, Redundant Operations \\
\midrule
 & Memory & Dynamic Resizing (Lack of prealloacation), Redundant Code, Inefficient Data Handling \\

\hline
\end{tabular}
\end{table*}

==> Tables/Optimization-Baseline-LLMs.tex <==
\begin{landscape}
\begin{table}
\centering
		\caption{Energy Optimization of code suggested by LLMs \pr{Show the delta for other columns, compared to Baseline}}
  \label{tab:optimization-baseline-llms}
		\begin{tabular}{l|rrrr|rrrr|rrrr|}			
  \toprule
        \multirow{2}{*}{\textbf{Project/File}} & \multicolumn{4}{|c|}{\textbf{Execution Time}} & \multicolumn{4}{|c|}{\textbf{Used Memory (MB)}} & \multicolumn{4}{|c|}{\textbf{CPU-Energy (kJ}} \\
        & \textbf{Baseline} & \textbf{GPT-3} & \textbf{GPT-4} & \textbf{Mixtral} & \textbf{Baseline} & \textbf{GPT-3} & \textbf{GPT-4} & \textbf{Mixtral} & \textbf{Baseline} & \textbf{GPT-3} & \textbf{GPT-4} & \textbf{Mixtral} \\
     \midrule
     UCI-DataSets-monks1D & 28.63 & 28.63 & 28.63 & & 37583.83 & 37580.58 & 37590.94 & & 109173.02 & 109095.24 & 109122.05 &  \\
PSO-basic-main & 28.63 & 28.63 & 28.63 & & 37583.41 & 37580.13 & 37558.41  & & 109058.26 & 109161.63 & 109116.32 & \\
private-getEnvironment & 28.60 & 28.63 & 28.63 & & 37591.24 &  37582.94  & 37583.87  & & 109080.45 & 109165.91 & 109130.76 &  \\
fetch-region-proposals & 28.63 & 28.63 & 28.63 & & 37961.4 & 37903.17 & 37803.42  & & 109088.52 & 109080.49 & 109094.74 & \\ 
afni-Test-m3dReorder & 28.63 & 28.63 & 28.63 & & 37582.13 & 37574.88 & 37595.78 & & 109172.56 & 109138.02 & 109153.42 & \\
\hline
\end{tabular}
\end{table}
\end{landscape}
